Return to Tradition: Learning Reliable Heuristics with Classical Machine Learning

Current approaches for learning for planning have yet to achieve competitive performance against classical planners in several domains, and have poor overall performance. In this work, we construct novel graph representations of lifted planning tasks and use the WL algorithm to generate features from them. These features are used with classical machine learning methods which have up to 2 orders of magnitude fewer parameters and train up to 3 orders of magnitude faster than the state-of-the-art deep learning for planning models. Our novel approach, WL-GOOSE, reliably learns heuristics from scratch and outperforms the $h^{\text{FF}}$ heuristic in a fair competition setting. It also outperforms or ties with LAMA on 4 out of 10 domains on coverage and 7 out of 10 domains on plan quality. WL-GOOSE is the first learning for planning model which achieves these feats. Furthermore, we study the connections between our novel WL feature generation method, previous theoretically flavoured learning architectures, and Description Logic Features for planning.

==> figures/experimental_results.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\centering
\tablesize
\caption{  
Coverage of domain-independent planners and domain-dependent learners.
%
The bottom-most row provides the overall IPC 2023 learning track score.
%
Our new models are the WL models.
%
The best entry in each row is highlighted in \textbf{bold}, and the top three
planners are indicated by the cell colouring intensity.  
%
}\label{tab:summary}
\input{tables/summarised_solved_quality.tex}
\end{table}

\newcommand{\cumulativewidth}{0.4\columnwidth}
\begin{figure}[t]
\centering
\raisebox{-0.5\height}{\includegraphics[width=\cumulativewidth]{figures/cumulative_runtime.pdf}}
\raisebox{-0.5\height}{\includegraphics[width=\cumulativewidth]{figures/cumulative_expanded.pdf}}
\raisebox{-0.4\height}{\includegraphics[width=0.15\columnwidth]{figures/cumulative_legend-cropped.pdf}}
\caption{  
Cumulative runtime in seconds (left) and node expansions (right) of planners.  
%
Domain-independent heuristics have solid linestyle, GNN methods have dotted
linestyle, and WL-GOOSE models have dashed linestyle. 
%
% \Todo{}: fix legend 
%
}
\end{figure}

\newcommand{\smlversuswidth}{0.39\columnwidth}
\begin{figure}[t]
\centering
\raisebox{-0.5\height}{\includegraphics[width=\smlversuswidth]{figures/cost_1wl_4_gp_none_vs_hff.pdf}}
\raisebox{-0.5\height}{\includegraphics[width=\smlversuswidth]{figures/expanded_1wl_4_gp_none_vs_hff.pdf}}
\raisebox{-0.45\height}{\includegraphics[width=0.2\columnwidth]{figures/versus_legend.pdf}}
\caption{Returned plan cost and number of expanded nodes of \hff{} and \gpr{}.
%
Problems that were not solved by one planner has their respective metric set to
the axis limit.
%
Points on the top left triangle favour \gpr{} while points on the bottom right
triangle favour \hff{}.
%
}
\label{fig:gpr_vs_hff}
\end{figure}


==> tables/benchmarks.tex <==
\begin{table*}
    \centering
    \caption{  
    Sizes of problems in the easy, medium and hard difficulties of each domain in
    the IPC 2023 Learning Track benchmarks~\cite{seipp:segovia:2023}. 
    %
    Training problems have size in the easy category.  
    }\label{tab:sizes}
    \small
    \begin{tabularx}{\textwidth}{X X X X X}
    \toprule
    % & & \multicolumn{3}{l}{Difficulty sizes} \\
    Domain & Objects & Easy & Medium & Hard \\
    \midrule 
    Blocksworld & $b$ blocks & $b \in [5, 30]$ & $b \in [35, 150]$ & $b \in [160,
    500]$ \\  
    \midrule 
    Childsnack  
    & $s$ sandwiches & $s \in [4, 15]$ & $s \in [15, 60]$ & $s \in [50, 450]$ \\ 
    & $c$ children & $c \in [4, 10]$ & $c \in [15, 40]$& $c \in [50, 300]$\\  
    & $t$ trays & $t \in [1, 3]$ & $t \in [2, 5]$ & $t \in [4, 10]$\\
    \midrule 
    Ferry  
    & $c$ cars & $c \in [1, 20]$ & $c \in [10, 100]$ & $c \in [200, 1000]$ \\
    & $l$ locations & $l \in [5, 15]$ & $l \in [20, 50]$ & $l \in [100, 500]$ \\
    \midrule 
    Floortile  
    & $n$ grid size & $n \in [3, 8]$ & $n \in [10, 22]$ & $n \in [25, 37]$ \\
    & $r$ robots & $r \in [1, 3]$ & $r \in [4, 15]$ & $r \in [15, 35]$ \\
    \midrule 
    Miconic  
    & $p$ passengers & $p \in [1, 10]$ & $p \in [20, 80]$ & $p \in [50, 500]$ \\
    & $f$ floors & $f \in [4, 20]$ & $f \in [30, 60]$ & $f \in [80, 200]$ \\
    \midrule 
    Rovers  
    & $r$ rovers & $r \in [1, 4]$ & $r \in [5, 10]$ & $r \in [15, 30]$ \\
    & $o$ objectives & $o \in [1, 10]$ & $o \in [15, 80]$ & $o \in [100, 200]$ \\
    & $c$ cameras & $c \in [1, 4]$ & $c \in [5, 50]$ & $c \in [60, 100]$ \\
    & $w$ waypoints & $w \in [4, 10]$ & $w \in [15, 90]$ & $w \in [100, 200]$ \\
    \midrule 
    Satellite  
    & $s$ satellites & $s \in [3, 10]$ & $s \in [15, 40]$ & $s \in [50, 100]$ \\
    & $i$ instruments & $i \in [3, 20]$ & $i \in [15, 80]$ & $i \in [50, 200]$ \\
    & $m$ modes & $m \in [1, 3]$ & $m \in [3, 5]$ & $m \in [5, 10]$  \\
    & $d$ directions & $d \in [4, 10]$ & $d \in [15, 30]$ & $d \in [40, 100]$ \\
    \midrule 
    Sokoban  
    & $n$ grid size & $n \in [8, 13]$ & $n \in [20, 50]$ & $n \in [60, 100]$ \\
    & $b$ boxes & $b \in [1, 4]$ & $b \in [5, 35]$ & $b \in [40, 80]$ \\
    \midrule
    Spanner  
    & $l$ locations & $l \in [4, 10]$ & $l \in [15, 45]$ & $l \in [50, 100]$ \\
    & $s$ spanners & $s \in [1, 10]$ & $s\in [30, 90]$ & $s \in [100, 500]$ \\
    & $n$ nuts & $n \in [1, 5]$ & $n \in [15, 50]$ & $n \in [50, 250]$ \\
    \midrule
    Transport  
    & $p$ packages & $p \in [1, 15]$ & $p \in [5, 45]$ & $p \in [20, 200]$ \\
    & $l$ locations &  $l \in [5, 15]$ & $l \in [20, 40]$ & $l \in [50, 100]$ \\
    & $v$ vehicles & $v \in [3, 6]$ & $v \in [10, 20]$ & $v \in [30, 50]$ \\
    & $m$ capacity & $m=2$ & $m=4$ & $m=10$\\
    \bottomrule 
    \end{tabularx}
    \end{table*}
    

==> tables/correlation_without_ratio.tex <==
blocksworld & \significant{\highcorr{+0.92}} & \significant{\highcorr{+0.91}} & \significant{\highcorr{+0.93}} & \significant{\highcorr{+0.98}} & \notsignificant{\medcorr{+0.34}} & \notsignificant{\lowcorr{-0.06}} & \significant{\highcorr{+0.79}} & \notsignificant{\lowcorr{+0.06}}\\
childsnack & \significant{\highcorr{+0.55}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \significant{\highcorr{+0.55}} & \significant{\highcorr{+0.68}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \significant{\highcorr{+0.68}}\\
ferry & \significant{\highcorr{+0.86}} & \significant{\highcorr{+0.98}} & \significant{\highcorr{+0.98}} & \significant{\highcorr{+1.00}} & \significant{\highcorr{+0.88}} & \significant{\highcorr{+0.88}} & \significant{\highcorr{+0.53}} & \significant{\highcorr{+0.83}}\\
floortile & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}\\
miconic & \significant{\highcorr{+0.56}} & \significant{\highcorr{+0.68}} & \significant{\highcorr{+0.97}} & \significant{\highcorr{+0.96}} & \significant{\highcorr{+0.56}} & \significant{\highcorr{+0.77}} & \significant{\highcorr{+0.99}} & \significant{\highcorr{+0.99}}\\
rovers & \significant{\highcorr{+0.88}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \significant{\highcorr{+0.95}} & \notsignificant{\lowcorr{+0.26}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \significant{\highcorr{+0.59}}\\
satellite & \significant{\highcorr{+0.73}} & \significant{\highcorr{+0.94}} & \multicolumn{1}{c}{-} & \significant{\highcorr{+0.96}} & \notsignificant{\lowcorr{+0.08}} & \notsignificant{\lowcorr{-0.24}} & \multicolumn{1}{c}{-} & \notsignificant{\lowcorr{+0.02}}\\
sokoban & \notsignificant{\lowcorr{+0.23}} & \significant{\highcorr{+0.83}} & \multicolumn{1}{c}{-} & \significant{\highcorr{+0.95}} & \notsignificant{\lowcorr{+0.25}} & \significant{\highcorr{+0.72}} & \multicolumn{1}{c}{-} & \significant{\highcorr{+0.79}}\\
spanner & \significant{\highcorr{+0.80}} & \significant{\highcorr{+0.53}} & \significant{\highcorr{+0.96}} & \significant{\highcorr{+0.92}} & \significant{\highcorr{+0.83}} & \significant{\highcorr{+0.54}} & \significant{\highcorr{+0.96}} & \significant{\highcorr{+0.92}}\\
transport & \significant{\highcorr{+0.83}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \significant{\highcorr{+0.83}} & \notsignificant{\lowcorr{+0.24}} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \notsignificant{\lowcorr{+0.25}}\\
\bottomrule


==> tables/features.tex <==
\begin{table}
    \centering
    \caption{\Todo{}}
    \label{tab:blocksworld}
    \tablesize
    \begin{tabularx}{\columnwidth}{l l}
        \toprule
        Weight & Features and Semantic Meaning \\
        \midrule
        -1.80 &  \\
        % -1.802952 & \\
        & $4406 = \hash(406,\mset{(4385,0)})$ \\
        & $4417 = \hash(4394,\mset{(4384,1),(4390,0)})$ \\
        & $4429 = \hash(421,\mset{(4384,0),(4389,1)})$ \\
        & $4439 = \hash(884,\mset{(4385,1),(4392,0)})$ \\
        & $4397 = \hash(4385,\mset{(406,0),(881,0),(884,1),(929,0)})$ \\
        & $4414 = \hash(81,\mset{(1727,1),(4242,0)})$ \\
        & $4384 = \hash(357,\mset{(372,0),(377,0),(382,1),(4382,1)})$ \\
        & $4385 = \hash(360,\mset{(362,0),(866,0),(869,1),(918,0)})$ \\
        & $4422 = \hash(416,\mset{(4384,0)})$ \\
        & $4430 = \hash(881,\mset{(1727,1),(4385,0)})$ \\
        & $4435 = \hash(420,\mset{(4389,0),(4392,1)})$ \\
        & $4396 = \hash(4384,\mset{(416,0),(421,0),(426,1),(4394,1)})$ \\
        -1.70 & \\
        % -1.696948 & \\
       & $49 = \hash(23,\mset{(10,0)})$ \\
       & $85 = \hash(49,\mset{(28,0)})$ \\
       & $28 = \hash(10,\mset{(21,1),(23,0)})$ \\
       & $10 = \hash(0,\mset{(3,1),(5,0)})$ \\
       \phantom{-}1.67 & \\
    %    1.670560 & \\
       & $8547 = \hash(422,\mset{(1654,0),(8532,1)})$ \\
       & $8534 = \hash(8532,\mset{(410,1),(414,0),(422,1),(674,0)})$ \\
       & $8542 = \hash(420,\mset{(1419,1),(5287,0)})$ \\
       & $8532 = \hash(35,\mset{(366,1),(370,0),(378,1),(658,0)})$ \\
       & $8544 = \hash(426,\mset{(668,1),(8533,0)})$ \\
       & $8539 = \hash(407,\mset{(715,0),(8533,1)})$ \\
       & $8540 = \hash(410,\mset{(1060,0),(3501,1)})$ \\
       & $8541 = \hash(422,\mset{(1654,1),(3501,0)})$ \\
       & $8543 = \hash(674,\mset{(663,1),(8532,0)})$ \\
       & $8537 = \hash(414,\mset{(668,1),(8532,0)})$ \\
       & $8538 = \hash(410,\mset{(5287,1),(8533,0)})$ \\
       & $8535 = \hash(8533,\mset{(407,1),(410,0),(422,1),(426,0)})$ \\
       & $8545 = \hash(90,\mset{(715,0),(5287,1)})$ \\
       & $8533 = \hash(35,\mset{(363,1),(366,0),(378,1),(382,0)})$ \\
       & $8546 = \hash(422,\mset{(1060,0),(8533,1)})$ \\
       & $8536 = \hash(410,\mset{(5287,0),(8532,1)})$ \\
        \bottomrule
    \end{tabularx}
\end{table}


==> tables/new_only_quality.tex <==
\begin{tabularx}{\columnwidth}{lX X X X X X} \toprule 
& \multicolumn{4}{c}{kernel} & \multicolumn{1}{c}{WLF} & \multicolumn{1}{c}{Bayes.} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
Domain 
& \header{\svrOne} 
& \header{\svrTwo} 
& \header{\svrThree} 
& \header{\svrInf} 
& \header{\lwlTwo} 
& \header{\gpr} 
\\ \midrule
blocksworld
& \first{44.4}{} & \third{20.2}{} & \normalcell{14.2}{} & \normalcell{17.8}{} & \normalcell{11.7}{} & \second{43.5}{} \\ 
childsnack
& \second{18.9}{} & \normalcell{11.5}{} & \normalcell{10.8}{} & \normalcell{13.5}{} & \third{16.6}{} & \first{19.4}{} \\ 
ferry
& \second{73.6}{} & \third{61.5}{} & \normalcell{35.4}{} & \normalcell{26.2}{} & \normalcell{59.6}{} & \first{75.6}{} \\ 
floortile
& \first{1.8}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{1.8}{} \\ 
miconic
& \second{89.0}{} & \third{86.9}{} & \normalcell{28.8}{} & \normalcell{28.7}{} & \normalcell{61.4}{} & \first{89.1}{} \\ 
rovers
& \second{36.4}{} & \normalcell{26.6}{} & \normalcell{26.2}{} & \normalcell{21.8}{} & \third{26.9}{} & \first{37.9}{} \\ 
satellite
& \first{32.9}{} & \normalcell{19.1}{} & \normalcell{16.0}{} & \normalcell{17.7}{} & \third{24.9}{} & \second{32.0}{} \\ 
sokoban
& \second{33.1}{} & \normalcell{29.7}{} & \third{31.7}{} & \normalcell{24.7}{} & \normalcell{27.6}{} & \first{34.8}{} \\ 
spanner
& \normalcell{27.6}{} & \third{28.0}{} & \third{28.0}{} & \third{28.0}{} & \first{49.9}{} & \second{37.1}{} \\ 
transport
& \second{46.3}{} & \normalcell{29.6}{} & \normalcell{29.1}{} & \normalcell{21.8}{} & \third{31.8}{} & \first{46.9}{} \\ 
\midrule
sum
& \second{404.0}{} & \third{313.0}{} & \normalcell{220.2}{} & \normalcell{200.2}{} & \normalcell{310.3}{} & \first{417.9}{} \\ 
\bottomrule\end{tabularx}

==> tables/new_only_solved.tex <==
\begin{tabularx}{\columnwidth}{lX X X X X X} \toprule 
& \multicolumn{4}{c}{kernel} & \multicolumn{1}{c}{WLF} & \multicolumn{1}{c}{Bayes.} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-6}
\cmidrule(lr){7-7}
Domain 
& \header{\svrOne} 
& \header{\svrTwo} 
& \header{\svrThree} 
& \header{\svrInf} 
& \header{\lwlTwo} 
& \header{\gpr} 
\\ \midrule
blocksworld
& \first{73}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \second{72}{} \\ 
childsnack
& \second{16}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{20}{} \\ 
ferry
& \first{77}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \second{75}{} \\ 
floortile
& \first{2}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{2}{} \\ 
miconic
& \first{90}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{90}{} \\ 
rovers
& \first{36}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \second{34}{} \\ 
satellite
& \second{46}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{56}{} \\ 
sokoban
& \first{38}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{38}{} \\ 
spanner
& \first{74}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{74}{} \\ 
transport
& \second{29}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{30}{} \\ 
\midrule
sum
& \second{481}{} & \third{-}{} & \third{-}{} & \third{-}{} & \third{-}{} & \first{491}{} \\ 
\bottomrule\end{tabularx}

==> tables/relaxed_quality.tex <==
\begin{tabularx}{\columnwidth}{lX X X X X} \toprule 
& \multicolumn{3}{c}{single-queue} & \multicolumn{2}{c}{multi-queue} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-6}
Domain 
& \header{\mip} 
& \header{\svrOne} 
& \header{\gpr} 
& \header{\svrMq} 
& \header{\gprMq} 
\\ \midrule
blocksworld
& \normalcell{8.0}{} & \first{44.4}{} & \third{43.5}{} & \first{44.4}{} & \third{43.5}{} \\ 
childsnack
& \normalcell{18.0}{} & \third{18.9}{} & \second{19.4}{} & \normalcell{17.5}{ (-1.4)} & \first{21.1}{ (+1.7)} \\ 
ferry
& \third{75.6}{} & \normalcell{73.6}{} & \third{75.6}{} & \first{76.7}{ (+3.1)} & \second{75.7}{ (+0.1)} \\ 
floortile
& \first{1.8}{} & \first{1.8}{} & \first{1.8}{} & \first{1.8}{} & \first{1.8}{} \\ 
miconic
& \normalcell{88.5}{} & \normalcell{89.0}{} & \third{89.1}{} & \second{89.3}{ (+0.3)} & \first{89.4}{ (+0.3)} \\ 
rovers
& \normalcell{34.9}{} & \normalcell{36.4}{} & \third{37.9}{} & \first{40.6}{ (+4.2)} & \second{39.8}{ (+1.9)} \\ 
satellite
& \normalcell{23.3}{} & \third{32.9}{} & \normalcell{32.0}{} & \second{39.0}{ (+6.1)} & \first{40.1}{ (+8.1)} \\ 
sokoban
& \normalcell{27.0}{} & \third{33.1}{} & \first{34.8}{} & \third{33.1}{} & \first{34.8}{} \\ 
spanner
& \first{69.9}{} & \normalcell{27.6}{} & \normalcell{37.1}{} & \third{68.1}{ (+40.5)} & \second{69.0}{ (+31.9)} \\ 
transport
& \second{48.3}{} & \normalcell{46.3}{} & \normalcell{46.9}{} & \first{49.7}{ (+3.4)} & \third{48.2}{ (+1.3)} \\ 
\midrule
sum
& \normalcell{395.4}{} & \normalcell{404.0}{} & \third{417.9}{} & \second{460.2}{ (+56.2)} & \first{463.4}{ (+45.5)} \\ 
\bottomrule\end{tabularx}

==> tables/relaxed_solved.tex <==
\begin{tabularx}{\columnwidth}{lX X X X X} \toprule 
& \multicolumn{3}{c}{single-queue} & \multicolumn{2}{c}{multi-queue} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-6}
Domain 
& \header{\mip} 
& \header{\svrOne} 
& \header{\gpr} 
& \header{\svrMq} 
& \header{\gprMq} 
\\ \midrule
blocksworld
& \normalcell{8}{} & \first{73}{} & \third{72}{} & \first{73}{} & \third{72}{} \\ 
childsnack
& \third{18}{} & \normalcell{16}{} & \second{20}{} & \third{18}{ (+2)} & \first{22}{ (+2)} \\ 
ferry
& \first{77}{} & \first{77}{} & \normalcell{75}{} & \first{77}{} & \first{77}{ (+2)} \\ 
floortile
& \first{2}{} & \first{2}{} & \first{2}{} & \first{2}{} & \first{2}{} \\ 
miconic
& \first{90}{} & \first{90}{} & \first{90}{} & \first{90}{} & \first{90}{} \\ 
rovers
& \normalcell{24}{} & \first{36}{} & \third{34}{} & \second{35}{ (-1)} & \third{34}{} \\ 
satellite
& \normalcell{24}{} & \normalcell{46}{} & \second{56}{} & \third{52}{ (+6)} & \first{60}{ (+4)} \\ 
sokoban
& \normalcell{27}{} & \first{38}{} & \first{38}{} & \first{38}{} & \first{38}{} \\ 
spanner
& \first{74}{} & \first{74}{} & \first{74}{} & \first{74}{} & \first{74}{} \\ 
transport
& \second{48}{} & \normalcell{29}{} & \normalcell{30}{} & \first{50}{ (+21)} & \second{48}{ (+18)} \\ 
\midrule
sum
& \normalcell{392}{} & \normalcell{481}{} & \third{491}{} & \second{509}{ (+28)} & \first{517}{ (+26)} \\ 
\bottomrule\end{tabularx}

==> tables/short.tex <==
% \newcommand{\allfirst}[1]{\leavevmode\color{red}\textbf{#1}}
% \newcommand{\allfirst}[1]{\underline{\textbf{#1}}}
\newcommand{\allfirst}[1]{{\underline{#1}}}
% \renewcommand{\first}[2]{\cellcolor{\colorofcell!30}{{{#1}}\comparisonentry{#2}}}

\begin{tabularx}{\columnwidth}{l r r r} \toprule 
    Domain 
    & \header{\ff} 
    & \header{GOOSE} 
    & \header{WL-GOOSE} 
    \\ \midrule
    blocksworld & \normalcell{28}{}& \second{63.0}{} & \first{{77}}{}\\
    childsnack & \second{26}{} & \normalcell{23.2}{} & \first{30}{}\\
    ferry & \normalcell{68}{} &\second{70.0}{}& \first{76}{}\\
    floortile & \first{{12}}{}& \normalcell{0.0}{}& \second{2}{}\\
    miconic & \first{{90}}{} &\normalcell{88.6}{} &\first{{90}}{}\\
    rovers & \second{34}{} & \normalcell{25.6}{} & \first{37}{}\\
    satellite & \first{65}{} & \normalcell{31.0}{} & \second{57}{}\\
    sokoban & \third{36}{} & \normalcell{33.0}{} & \first{38}{}\\
    spanner & \normalcell{30}{} & \second{46.4}{} & \first{\allfirst{74}}{}\\
    transport & \first{41}{} & \second{32.4}{} & \normalcell{32}{}\\
    \midrule
    sum coverage
    & \third{430}{} & \normalcell{413.2}{} & \first{513}{}\\
    sum IPC score
    & \third{393.5}{} & \normalcell{391.0}{} & \first{471.2}{}\\
    \bottomrule\end{tabularx}


==> tables/summarised_lama_quality.tex <==
\begin{tabularx}{\columnwidth}{l Y Y Y Y Y Y Y Y Y} \toprule 
Domain 
& \header{\lama} 
& \header{\ff} 
& \header{\muninn} 
& \header{\gooseMax} 
& \header{\gooseMean} 
& \header{\svrOne} 
& \header{\svrInf} 
& \header{\lwlTwo} 
& \header{\gprNew} 
\\ \midrule
blocksworld
& \normalcell{39.8}{} & \normalcell{14.1}{} & \normalcell{40.0}{} & \normalcell{45.6}{} & \third{52.7}{} & \second{66.1}{} & \normalcell{19.2}{} & \normalcell{14.2}{} & \first{70.2}{} \\ 
childsnack
& \normalcell{22.0}{} & \second{20.1}{} & \normalcell{11.0}{} & \normalcell{17.6}{} & \third{19.9}{} & \normalcell{15.1}{} & \normalcell{12.6}{} & \normalcell{10.8}{} & \first{27.8}{} \\ 
ferry
& \normalcell{62.9}{} & \normalcell{67.6}{} & \normalcell{46.0}{} & \normalcell{63.9}{} & \third{71.9}{} & \first{76.9}{} & \normalcell{30.8}{} & \normalcell{59.6}{} & \second{75.8}{} \\ 
floortile
& \normalcell{10.0}{} & \first{11.2}{} & \normalcell{-}{} & \normalcell{-}{} & \normalcell{-}{} & \second{1.8}{} & \normalcell{-}{} & \normalcell{0.9}{} & \second{1.8}{} \\ 
miconic
& \normalcell{81.6}{} & \normalcell{88.5}{} & \normalcell{30.0}{} & \first{89.2}{} & \second{89.1}{} & \third{88.9}{} & \normalcell{30.0}{} & \normalcell{66.0}{} & \normalcell{88.6}{} \\ 
rovers
& \normalcell{65.2}{} & \first{32.7}{} & \normalcell{14.2}{} & \normalcell{19.7}{} & \normalcell{24.8}{} & \third{26.6}{} & \normalcell{22.4}{} & \third{26.6}{} & \second{29.8}{} \\ 
satellite
& \normalcell{87.3}{} & \first{63.8}{} & \normalcell{18.0}{} & \normalcell{24.6}{} & \normalcell{21.6}{} & \third{36.8}{} & \normalcell{20.2}{} & \normalcell{17.2}{} & \second{47.8}{} \\ 
sokoban
& \normalcell{29.8}{} & \normalcell{26.3}{} & \normalcell{24.3}{} & \normalcell{28.3}{} & \third{30.0}{} & \first{34.7}{} & \normalcell{26.7}{} & \normalcell{28.4}{} & \first{34.7}{} \\ 
spanner
& \normalcell{30.0}{} & \normalcell{30.0}{} & \normalcell{32.0}{} & \normalcell{30.0}{} & \normalcell{33.0}{} & \first{70.0}{} & \normalcell{28.9}{} & \third{47.9}{} & \first{70.0}{} \\ 
transport
& \normalcell{64.0}{} & \first{39.3}{} & \normalcell{17.0}{} & \second{35.6}{} & \normalcell{31.6}{} & \normalcell{26.0}{} & \normalcell{22.8}{} & \third{33.2}{} & \normalcell{24.8}{} \\ 
\midrule
sum
& \normalcell{492.7}{} & \third{393.5}{} & \normalcell{232.4}{} & \normalcell{354.5}{} & \normalcell{374.6}{} & \second{442.8}{} & \normalcell{213.4}{} & \normalcell{304.8}{} & \first{471.2}{} \\ 
\bottomrule\end{tabularx}

==> tables/summarised_lama_solved.tex <==
\begin{tabularx}{\columnwidth}{l Y Y Y Y Y Y Y Y Y} \toprule 
Domain 
& \header{\lama} 
& \header{\ff} 
& \header{\muninn} 
& \header{\gooseMax} 
& \header{\gooseMean} 
& \header{\svrOne} 
& \header{\svrInf} 
& \header{\lwlTwo} 
& \header{\gprNew} 
\\ \midrule
blocksworld
& \normalcell{61}{} & \normalcell{28}{} & \normalcell{40}{} & \normalcell{49}{} & \third{58}{} & \second{72}{} & \normalcell{20}{} & \normalcell{22}{} & \first{77}{} \\ 
childsnack
& \normalcell{35}{} & \second{26}{} & \normalcell{11}{} & \normalcell{19}{} & \third{20}{} & \normalcell{16}{} & \normalcell{15}{} & \normalcell{13}{} & \first{30}{} \\ 
ferry
& \normalcell{68}{} & \normalcell{68}{} & \normalcell{46}{} & \normalcell{64}{} & \third{72}{} & \first{77}{} & \normalcell{32}{} & \normalcell{60}{} & \second{76}{} \\ 
floortile
& \normalcell{11}{} & \first{12}{} & \normalcell{-}{} & \normalcell{-}{} & \normalcell{-}{} & \second{2}{} & \normalcell{-}{} & \normalcell{1}{} & \second{2}{} \\ 
miconic
& \first{90}{} & \first{90}{} & \normalcell{30}{} & \first{90}{} & \first{90}{} & \first{90}{} & \normalcell{31}{} & \normalcell{67}{} & \first{90}{} \\ 
rovers
& \normalcell{67}{} & \second{34}{} & \normalcell{15}{} & \normalcell{25}{} & \normalcell{29}{} & \third{33}{} & \normalcell{27}{} & \third{33}{} & \first{37}{} \\ 
satellite
& \normalcell{89}{} & \first{65}{} & \normalcell{18}{} & \normalcell{31}{} & \normalcell{29}{} & \third{46}{} & \normalcell{29}{} & \normalcell{20}{} & \second{57}{} \\ 
sokoban
& \normalcell{40}{} & \third{36}{} & \normalcell{26}{} & \normalcell{32}{} & \normalcell{33}{} & \first{38}{} & \normalcell{30}{} & \normalcell{31}{} & \first{38}{} \\ 
spanner
& \normalcell{30}{} & \normalcell{30}{} & \normalcell{32}{} & \normalcell{30}{} & \normalcell{33}{} & \first{74}{} & \normalcell{30}{} & \third{52}{} & \first{74}{} \\ 
transport
& \normalcell{66}{} & \first{41}{} & \normalcell{17}{} & \second{38}{} & \third{35}{} & \normalcell{29}{} & \normalcell{26}{} & \third{35}{} & \normalcell{32}{} \\ 
\midrule
sum
& \normalcell{557}{} & \third{430}{} & \normalcell{235}{} & \normalcell{378}{} & \normalcell{399}{} & \second{477}{} & \normalcell{240}{} & \normalcell{334}{} & \first{513}{} \\ 
\bottomrule\end{tabularx}

==> tables/summarised_quality.tex <==
\begin{tabularx}{\columnwidth}{l Y Y Y Y Y Y Y Y Y} \toprule 
Domain 
& \header{\blind} 
& \header{\ff} 
& \header{\muninn} 
& \header{\gooseMax} 
& \header{\gooseMean} 
& \header{\svrOne} 
& \header{\svrInf} 
& \header{\lwlTwo} 
& \header{\gprNew} 
\\ \midrule
blocksworld
& \normalcell{8.0}{} & \normalcell{14.1}{} & \normalcell{40.0}{} & \normalcell{45.6}{} & \third{52.7}{} & \second{66.1}{} & \normalcell{19.2}{} & \normalcell{14.2}{} & \first{70.2}{} \\ 
childsnack
& \normalcell{9.0}{} & \second{20.1}{} & \normalcell{11.0}{} & \normalcell{17.6}{} & \third{19.9}{} & \normalcell{15.1}{} & \normalcell{12.6}{} & \normalcell{10.8}{} & \first{27.8}{} \\ 
ferry
& \normalcell{10.0}{} & \normalcell{67.6}{} & \normalcell{46.0}{} & \normalcell{63.9}{} & \third{71.9}{} & \first{76.9}{} & \normalcell{30.8}{} & \normalcell{59.6}{} & \second{75.8}{} \\ 
floortile
& \second{2.0}{} & \first{11.2}{} & \normalcell{-}{} & \normalcell{-}{} & \normalcell{-}{} & \third{1.8}{} & \normalcell{-}{} & \normalcell{0.9}{} & \third{1.8}{} \\ 
miconic
& \normalcell{30.0}{} & \normalcell{88.5}{} & \normalcell{30.0}{} & \first{89.2}{} & \second{89.1}{} & \third{88.9}{} & \normalcell{30.0}{} & \normalcell{66.0}{} & \normalcell{88.6}{} \\ 
rovers
& \normalcell{15.0}{} & \first{32.7}{} & \normalcell{14.2}{} & \normalcell{19.7}{} & \normalcell{24.8}{} & \third{26.6}{} & \normalcell{22.4}{} & \third{26.6}{} & \second{29.8}{} \\ 
satellite
& \normalcell{12.0}{} & \first{63.8}{} & \normalcell{18.0}{} & \normalcell{24.6}{} & \normalcell{21.6}{} & \third{36.8}{} & \normalcell{20.2}{} & \normalcell{17.2}{} & \second{47.8}{} \\ 
sokoban
& \normalcell{27.0}{} & \normalcell{26.3}{} & \normalcell{24.3}{} & \normalcell{28.3}{} & \third{30.0}{} & \first{34.7}{} & \normalcell{26.7}{} & \normalcell{28.4}{} & \first{34.7}{} \\ 
spanner
& \normalcell{30.0}{} & \normalcell{30.0}{} & \normalcell{32.0}{} & \normalcell{30.0}{} & \normalcell{33.0}{} & \first{70.0}{} & \normalcell{28.9}{} & \third{47.9}{} & \first{70.0}{} \\ 
transport
& \normalcell{9.0}{} & \first{39.3}{} & \normalcell{17.0}{} & \second{35.6}{} & \normalcell{31.6}{} & \normalcell{26.0}{} & \normalcell{22.8}{} & \third{33.2}{} & \normalcell{24.8}{} \\ 
\midrule
sum
& \normalcell{152.0}{} & \third{393.5}{} & \normalcell{232.4}{} & \normalcell{354.5}{} & \normalcell{374.6}{} & \second{442.8}{} & \normalcell{213.4}{} & \normalcell{304.8}{} & \first{471.2}{} \\ 
\bottomrule\end{tabularx}

==> tables/summarised_solved.tex <==
\begin{tabularx}{\columnwidth}{l Y Y Y Y Y Y Y Y Y} \toprule 
Domain 
& \header{\blind} 
& \header{\ff} 
& \header{\muninn} 
& \header{\gooseMax} 
& \header{\gooseMean} 
& \header{\svrOne} 
& \header{\svrInf} 
& \header{\lwlTwo} 
& \header{\gprNew} 
\\ \midrule
blocksworld
& \normalcell{8}{} & \normalcell{28}{} & \normalcell{40}{} & \normalcell{49}{} & \third{58}{} & \second{72}{} & \normalcell{20}{} & \normalcell{22}{} & \first{77}{} \\ 
childsnack
& \normalcell{9}{} & \second{26}{} & \normalcell{11}{} & \normalcell{19}{} & \third{20}{} & \normalcell{16}{} & \normalcell{15}{} & \normalcell{13}{} & \first{30}{} \\ 
ferry
& \normalcell{10}{} & \normalcell{68}{} & \normalcell{46}{} & \normalcell{64}{} & \third{72}{} & \first{77}{} & \normalcell{32}{} & \normalcell{60}{} & \second{76}{} \\ 
floortile
& \second{2}{} & \first{12}{} & \normalcell{-}{} & \normalcell{-}{} & \normalcell{-}{} & \second{2}{} & \normalcell{-}{} & \normalcell{1}{} & \second{2}{} \\ 
miconic
& \normalcell{30}{} & \first{90}{} & \normalcell{30}{} & \first{90}{} & \first{90}{} & \first{90}{} & \normalcell{31}{} & \normalcell{67}{} & \first{90}{} \\ 
rovers
& \normalcell{15}{} & \second{34}{} & \normalcell{15}{} & \normalcell{25}{} & \normalcell{29}{} & \third{33}{} & \normalcell{27}{} & \third{33}{} & \first{37}{} \\ 
satellite
& \normalcell{12}{} & \first{65}{} & \normalcell{18}{} & \normalcell{31}{} & \normalcell{29}{} & \third{46}{} & \normalcell{29}{} & \normalcell{20}{} & \second{57}{} \\ 
sokoban
& \normalcell{27}{} & \third{36}{} & \normalcell{26}{} & \normalcell{32}{} & \normalcell{33}{} & \first{38}{} & \normalcell{30}{} & \normalcell{31}{} & \first{38}{} \\ 
spanner
& \normalcell{30}{} & \normalcell{30}{} & \normalcell{32}{} & \normalcell{30}{} & \normalcell{33}{} & \first{74}{} & \normalcell{30}{} & \third{52}{} & \first{74}{} \\ 
transport
& \normalcell{9}{} & \first{41}{} & \normalcell{17}{} & \second{38}{} & \third{35}{} & \normalcell{29}{} & \normalcell{26}{} & \third{35}{} & \normalcell{32}{} \\ 
\midrule
sum
& \normalcell{152}{} & \third{430}{} & \normalcell{235}{} & \normalcell{378}{} & \normalcell{399}{} & \second{477}{} & \normalcell{240}{} & \normalcell{334}{} & \first{513}{} \\ 
\bottomrule\end{tabularx}

==> tables/summarised_solved_quality.tex <==
\begin{tabularx}{\columnwidth}{lY Y Y Y Y Y Y Y Y} \toprule 
    &
    \multicolumn{2}{c}{classical} 
    &
    \multicolumn{3}{c}{GNN}
    &
    \multicolumn{4}{c}{WLF}
    \\
    \cmidrule(lr){2-3}  
    \cmidrule(lr){4-6}  
    \cmidrule(lr){7-10}  
    Domain 
    & \header{\blind} 
    & \header{\ff} 
    & \header{\muninn} 
    & \header{\gooseMax} 
    & \header{\gooseMean} 
    & \header{\svrOne} 
    & \header{\svrInf} 
    & \header{\lwlTwo} 
    & \header{\gprNew} 
    \\ \midrule
    blocksworld
    & \normalcell{8}{} & \normalcell{28}{} & \normalcell{40}{} & \normalcell{49}{} & \third{58}{} & \second{72}{} & \normalcell{20}{} & \normalcell{22}{} & \first{77}{} \\ 
    childsnack
    & \normalcell{9}{} & \second{26}{} & \normalcell{11}{} & \normalcell{19}{} & \third{20}{} & \normalcell{16}{} & \normalcell{15}{} & \normalcell{13}{} & \first{30}{} \\ 
    ferry
    & \normalcell{10}{} & \normalcell{68}{} & \normalcell{46}{} & \normalcell{64}{} & \third{72}{} & \first{77}{} & \normalcell{32}{} & \normalcell{60}{} & \second{76}{} \\ 
    floortile
    & \second{2}{} & \first{12}{} & \normalcell{-}{} & \normalcell{-}{} & \normalcell{-}{} & \second{2}{} & \normalcell{-}{} & \normalcell{1}{} & \second{2}{} \\ 
    miconic
    & \normalcell{30}{} & \first{90}{} & \normalcell{30}{} & \first{90}{} & \first{90}{} & \first{90}{} & \normalcell{31}{} & \normalcell{67}{} & \first{90}{} \\ 
    rovers
    & \normalcell{15}{} & \second{34}{} & \normalcell{15}{} & \normalcell{25}{} & \normalcell{29}{} & \third{33}{} & \normalcell{27}{} & \third{33}{} & \first{37}{} \\ 
    satellite
    & \normalcell{12}{} & \first{65}{} & \normalcell{18}{} & \normalcell{31}{} & \normalcell{29}{} & \third{46}{} & \normalcell{29}{} & \normalcell{20}{} & \second{57}{} \\ 
    sokoban
    & \normalcell{27}{} & \third{36}{} & \normalcell{26}{} & \normalcell{32}{} & \normalcell{33}{} & \first{38}{} & \normalcell{30}{} & \normalcell{31}{} & \first{38}{} \\ 
    spanner
    & \normalcell{30}{} & \normalcell{30}{} & \normalcell{32}{} & \normalcell{30}{} & \normalcell{33}{} & \first{74}{} & \normalcell{30}{} & \third{52}{} & \first{74}{} \\ 
    transport
    & \normalcell{9}{} & \first{41}{} & \normalcell{17}{} & \second{38}{} & \third{35}{} & \normalcell{29}{} & \normalcell{26}{} & \third{35}{} & \normalcell{32}{} \\ 
    \midrule
    sum coverage
    & \normalcell{152}{} & \third{430}{} & \normalcell{235}{} & \normalcell{378}{} & \normalcell{399}{} & \second{477}{} & \normalcell{240}{} & \normalcell{334}{} & \first{513}{} \\ 
    \midrule
    sum IPC score
    & \normalcell{152.0}{} & \third{393.5}{} & \normalcell{232.4}{} & \normalcell{354.5}{} & \normalcell{374.6}{} & \second{442.8}{} & \normalcell{213.4}{} & \normalcell{304.8}{} & \first{471.2}{} \\ 
    \bottomrule\end{tabularx}
